Measurement of the CKM angle alpha with the B-factories

B-meson decays involving b->u transitions are sensitive to the Unitarity Triangle angle alpha (or phi_2). The B-factories at SLAC and KEK have made significant progress toward the measurement of alpha in recent years. This paper summarizes the results of the B-factories' constraints on alpha.

==> babarsym.tex <==
%%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised   05/22/01 P. Dauncey     Added \hepex, etc. and clean up a bit
%%%%%   Revised   12/07/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised   07/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised   07/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised   07/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised   07/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised   07/01/00 D. MacFarlane
%%%%%   Revised   06/21/00 D. Hitlin
%%%%%   Original  06/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}}
\def\en         {\ensuremath{e^-}}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}}
\def\epm        {\ensuremath{e^\pm}} 
\def\epem       {\ensuremath{e^+e^-}}
\def\ee         {\ensuremath{e^-e^-}}

\def\mmu        {\ensuremath{\mu}}
\def\mup        {\ensuremath{\mu^+}}
\def\mun        {\ensuremath{\mu^-}} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}}
\def\mtau       {\ensuremath{\tau}}

\def\taup       {\ensuremath{\tau^+}}
\def\taum       {\ensuremath{\tau^-}}
\def\tautau     {\ensuremath{\tau^+\tau^-}}

\def\ellm       {\ensuremath{\ell^-}}
\def\ellp       {\ensuremath{\ell^+}}
\def\ellell     {\ensuremath{\ell^+ \ell^-}}

\def\nub        {\ensuremath{\overline{\nu}}}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}}
\def\nub        {\ensuremath{\overline{\nu}}}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}}
\def\nue        {\ensuremath{\nu_e}}
\def\nueb       {\ensuremath{\nub_e}}
\def\nuenueb    {\ensuremath{\nue\nueb}}
\def\num        {\ensuremath{\nu_\mu}}
\def\numb       {\ensuremath{\nub_\mu}}
\def\numnumb    {\ensuremath{\num\numb}}
\def\nut        {\ensuremath{\nu_\tau}}
\def\nutb       {\ensuremath{\nub_\tau}}
\def\nutnutb    {\ensuremath{\nut\nutb}}
\def\nul        {\ensuremath{\nu_\ell}}
\def\nulb       {\ensuremath{\nub_\ell}}
\def\nulnulb    {\ensuremath{\nul\nulb}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}}
\def\gaga  {\ensuremath{\gamma\gamma}}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}}

\def\ega    {\ensuremath{e\gamma}}
\def\game   {\ensuremath{\gamma e^-}}
\def\epemg  {\ensuremath{e^+e^-\gamma}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}}
\def\Hp     {\ensuremath{H^+}}
\def\Hm     {\ensuremath{H^-}}
\def\Hpm    {\ensuremath{H^\pm}}
\def\W      {\ensuremath{W}}
\def\Wp     {\ensuremath{W^+}}
\def\Wm     {\ensuremath{W^-}}
\def\Wpm    {\ensuremath{W^\pm}}
\def\Z      {\ensuremath{Z^0}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}}
\def\qbar  {\ensuremath{\overline q}}
\def\qqbar {\ensuremath{q\overline q}}
\def\u     {\ensuremath{u}}
\def\ubar  {\ensuremath{\overline u}}
\def\uubar {\ensuremath{u\overline u}}
\def\d     {\ensuremath{d}}
\def\dbar  {\ensuremath{\overline d}}
\def\ddbar {\ensuremath{d\overline d}}
\def\s     {\ensuremath{s}}
\def\sbar  {\ensuremath{\overline s}}
\def\ssbar {\ensuremath{s\overline s}}
\def\c     {\ensuremath{c}}
\def\cbar  {\ensuremath{\overline c}}
\def\ccbar {\ensuremath{c\overline c}}
\def\b     {\ensuremath{b}}
\def\bbar  {\ensuremath{\overline b}}
\def\bbbar {\ensuremath{b\overline b}}
\def\t     {\ensuremath{t}}
\def\tbar  {\ensuremath{\overline t}}
\def\tbar  {\ensuremath{\overline t}}
\def\ttbar {\ensuremath{t\overline t}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}}
\def\ppz   {\ensuremath{\pi^0\pi^0}}
\def\pip   {\ensuremath{\pi^+}}
\def\pim   {\ensuremath{\pi^-}}
\def\pipi  {\ensuremath{\pi^+\pi^-}}
\def\pipm  {\ensuremath{\pi^\pm}}
\def\pimp  {\ensuremath{\pi^\mp}}

\def\kaon  {\ensuremath{K}}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}}
\def\Kb    {\ensuremath{\Kbar}}
\def\Kz    {\ensuremath{K^0}}
\def\Kzb   {\ensuremath{\Kbar^0}}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}}
\def\Kp    {\ensuremath{K^+}}
\def\Km    {\ensuremath{K^-}}
\def\Kpm   {\ensuremath{K^\pm}}
\def\Kmp   {\ensuremath{K^\mp}}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}} 
\def\Kstarz  {\ensuremath{K^{*0}}}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}}
\def\Kstar   {\ensuremath{K^*}}
\def\Kstarb  {\ensuremath{\Kbar^*}}
\def\Kstarp  {\ensuremath{K^{*+}}}
\def\Kstarm  {\ensuremath{K^{*-}}}
\def\Kstarpm {\ensuremath{K^{*\pm}}}
\def\Kstarmp {\ensuremath{K^{*\mp}}}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}}
\def\Db      {\ensuremath{\Dbar}}
\def\Dz      {\ensuremath{D^0}}
\def\Dzb     {\ensuremath{\Dbar^0}}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}}
\def\Dp      {\ensuremath{D^+}}
\def\Dm      {\ensuremath{D^-}}
\def\Dpm     {\ensuremath{D^\pm}}
\def\Dmp     {\ensuremath{D^\mp}}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}}
\def\Dstar   {\ensuremath{D^*}}
\def\Dstarb  {\ensuremath{\Dbar^*}}
\def\Dstarz  {\ensuremath{D^{*0}}}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}}
\def\Dstarp  {\ensuremath{D^{*+}}}
\def\Dstarm  {\ensuremath{D^{*-}}}
\def\Dstarpm {\ensuremath{D^{*\pm}}}
\def\Dstarmp {\ensuremath{D^{*\mp}}}
\def\Ds      {\ensuremath{D^+_s}}
\def\Dsb     {\ensuremath{\Dbar^+_s}}
\def\Dss     {\ensuremath{D^{*+}_s}}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}}
\newcommand{\dstrstr}{\ensuremath{D^{**}}}
\newcommand{\dsp}{\ensuremath{\Dstarp}}
\newcommand{\dsm}{\ensuremath{\Dstarm}}
\newcommand{\dsz}{\ensuremath{\Dstarz}}


\def\B       {\ensuremath{B}}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}}
\def\Bb      {\ensuremath{\Bbar}}
\def\BB      {\ensuremath{B\Bbar}} 
\def\Bz      {\ensuremath{B^0}}
\def\Bzb     {\ensuremath{\Bbar^0}}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}}
\def\Bu      {\ensuremath{B^+}}
\def\Bub     {\ensuremath{B^-}}
\def\Bp      {\ensuremath{\Bu}}
\def\Bm      {\ensuremath{\Bub}}
\def\Bpm     {\ensuremath{B^\pm}}
\def\Bmp     {\ensuremath{B^\mp}}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}}
\def\Bs      {\ensuremath{B_s}}
\def\Bsb     {\ensuremath{\Bbar_s}}

% added by GHM on March 25, 2003 -- from Andrei Gritsan
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}}
\def\psitwos  {\ensuremath{\psi{(2S)}}}
\def\psiprpr  {\ensuremath{\psi(3770)}}
\def\etac     {\ensuremath{\eta_c}}
\def\chiczero {\ensuremath{\chi_{c0}}}
\def\chicone  {\ensuremath{\chi_{c1}}}
\def\chictwo  {\ensuremath{\chi_{c2}}}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}}
\def\antiproton  {\ensuremath{\overline p}}
\def\neutron     {\ensuremath{n}}
\def\antineutron {\ensuremath{\overline n}}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}}

\def\X {\ensuremath{X}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% TAU BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\cal B}}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}}

\def\BtoDK      {\ensuremath{B \to DK}}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}}

\def\Btoetah    {\ensuremath{B \to \eta h}}
\def\Btoetaph   {\ensuremath{B \to \etapr h}}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}}

\def\btosgam    {\ensuremath{b \to s \g}}
\def\btodgam    {\ensuremath{b \to d \g}}
\def\btosll     {\ensuremath{b \to s \ellell}}
\def\btosnunu   {\ensuremath{b \to s \nunub}}
\def\btosgaga   {\ensuremath{b \to s \gaga}}
\def\btosglue   {\ensuremath{b \to s g}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}}
%\def\pt         {\mbox{$p_{\rm t}$}}
\def\pt         {\mbox{$p_T$}}
\def\mes        {\mbox{$m_{\rm ES}$}}
\def\mec        {\mbox{$m_{\rm EC}$}}
\def\DeltaE     {\mbox{$\Delta E$}}

\def\pbcm {\ensuremath{p^*_{\Bz}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}}
\def\mtheta     {\mbox{$\theta$}}
\def\ctheta     {\mbox{$\cos\theta$}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}} 
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}} 
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}}
\def\inch   {\ensuremath{\rm \,in}} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}}
\def\km   {\ensuremath{{\rm \,km}}}
\def\m    {\ensuremath{{\rm \,m}}}
\def\cm   {\ensuremath{{\rm \,cm}}}
\def\cma  {\ensuremath{{\rm \,cm}^2}}
\def\mm   {\ensuremath{{\rm \,mm}}}
\def\mma  {\ensuremath{{\rm \,mm}^2}}
%\def\mum  {\ensuremath{{\rm \,\mum}}}
\def\mum  {\ensuremath{{\,\mu\rm m}}}%% mu meter 
%\def\muma {\ensuremath{\rm \,\mum}^2}
\def\muma       {\ensuremath{{\,\mu\rm m}^2}}
\def\nm   {\ensuremath{{\rm \,nm}}}
\def\fm   {\ensuremath{{\rm \,fm}}}
\def\nm         {\ensuremath{{\rm \,nm}}}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}}
\def\barnhyph{\ensuremath{{\rm -b}}}
\def\mbarn{\ensuremath{{\rm \,mb}}}
\def\mbarnhyph{\ensuremath{{\rm -mb}}}
\def\nb         {\ensuremath{{\rm \,nb}}}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}}
\def\pb {\ensuremath{{\rm \,pb}}}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}}
\def\fb   {\ensuremath{\mbox{\,fb}}}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}}
\def\ns   {\ensuremath{\rm \,ns}}
\def\ps   {\ensuremath{\rm \,ps}}
\def\fs   {\ensuremath{\rm \,fs}}
\def\gm   {\ensuremath{\rm \,g}}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}}
\def\NIL{\ensuremath{\lambda_{int}}}
\let\dgr\degrees


%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}


\def\mic  {\ensuremath{\,\mu{\rm C}}}
\def\krad {\ensuremath{\rm \,krad}}
\def\cmc  {\ensuremath{{\rm \,cm}^3}}
\def\yr   {\ensuremath{\rm \,yr}}
\def\hr   {\ensuremath{\rm \,hr}}
\def\degc {\ensuremath{^\circ}{C}}
\def\degk {\ensuremath {\rm K}}
\def\degrees{\ensuremath{^{\circ}}}
\def\mrad{\ensuremath{\rm \,mrad}}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}}
\def\mradhyph{\ensuremath{\rm -mr}}
%
\def\sx    {\ensuremath{\sigma_x}}    
\def\sy    {\ensuremath{\sigma_y}}   
\def\sz    {\ensuremath{\sigma_z}}    

%\renewcommand{\bar}[1]{\overline{#1}}  

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}}
\def\L{{\ensuremath{\cal L}}}
\def\calL{{\ensuremath{\cal L}}}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}}
\def\calA{{\ensuremath{\cal A}}}
\def\calD{{\ensuremath{\cal D}}}
\def\calR{{\ensuremath{\cal R}}}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}}
\def\to                 {\ensuremath{\rightarrow}}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}}


\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}}     
\def\sy    {\ensuremath{\sigma_y}}   
\def\sz    {\ensuremath{\sigma_z}}


\newcommand{\inverse}{\ensuremath{^{-1}}}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}}
\newcommand{\chisq}{\ensuremath{\chi^2}}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}}
\newcommand{\lum} {\ensuremath{\mathcal{L}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}}

\def\qsq                {\ensuremath{q^2}}


% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}}
\def\kbits      {\ensuremath{{\rm \,kbits}}}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}}
%




% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}}


% CKM, CP violation

\def\eps{\varepsilon}
\def\epsK{\varepsilon_K}
\def\epsB{\varepsilon_B}
\def\epsp{\varepsilon^\prime_K}

\def\CP                {\ensuremath{C\!P}}
%\def\CPT               {\ensuremath{C\!P\!T}}
\def\CPT               {\ensuremath{C\!PT}} % Looks better without \!
% added by GHM on March 25, 2003
\def\C       {\ensuremath{C}}
\def\P       {\ensuremath{P}}
\def\T       {\ensuremath{T}}



\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}}

\def\rhobar {\ensuremath{\overline \rho}}
\def\etabar {\ensuremath{\overline \eta}}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}}

\def\Vud  {\ensuremath{|V_{ud}|}}
\def\Vcd  {\ensuremath{|V_{cd}|}}
\def\Vtd  {\ensuremath{|V_{td}|}}
\def\Vus  {\ensuremath{|V_{us}|}}
\def\Vcs  {\ensuremath{|V_{cs}|}}
\def\Vts  {\ensuremath{|V_{ts}|}}
\def\Vub  {\ensuremath{|V_{ub}|}}
\def\Vcb  {\ensuremath{|V_{cb}|}}
\def\Vtb  {\ensuremath{|V_{tb}|}}

%\def\sa{${\sin\! 2 \alpha  }$}
%\def\sb{${\sin\! 2 \beta   }$}
%\def\sg{${\sin\! 2 \gamma  }$}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }}
\def\stwob{\ensuremath{\sin\! 2 \beta   }}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }}
\def\mistag{\ensuremath{w}}
\def\dilution{\ensuremath{\cal D}}
\def\deltaz{\ensuremath{{\rm \Delta}z}}
\def\deltat{\ensuremath{{\rm \Delta}t}}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}}

\newcommand{\fsubd}{\ensuremath{f_D}}
\newcommand{\fds}{\ensuremath{f_{D_s}}}
\newcommand{\fsubb}{\ensuremath{f_B}}
\newcommand{\fbd}{\ensuremath{f_{B_d}}}
\newcommand{\fbs}{\ensuremath{f_{B_s}}}
\newcommand{\bsubb}{\ensuremath{B_B}}
\newcommand{\bbd}{\ensuremath{B_{B_d}}}
\newcommand{\bbs}{\ensuremath{B_{B_s}}}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}






% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.}
\newcommand{\jprBase}        {Phys.\ Rev.}
\newcommand{\jplBase}        {Phys.\ Lett.}
%\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.}
%\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.}
%\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods}
%\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods}
%\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Meth.}
\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ A}
\newcommand{\nimBaseB}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ B}
\newcommand{\nimBaseC}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ C}
\newcommand{\nimBaseD}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ D}
\newcommand{\nimBaseE}       {Nucl.\ Instr.\ Methods Phys.\ Res., Sect.\ E}
\newcommand{\npBase}         {Nucl.\ Phys.}
\newcommand{\zpBase}         {Z.\ Phys.}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instrum.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimaa}       [1]  {\nimBaseE~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~{\bf #1}}
\newcommand{\nimb}      [1]  {\nimBaseB~{\bf #1}}
\newcommand{\nimc}      [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimd}      [1]  {\nimBaseD~{\bf #1}}
\newcommand{\nime}      [1]  {\nimBaseE~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}}
\def\bbsim      {\mbox{\tt BBsim}}
\def\beast      {\mbox{\tt Beast}}
\def\beget      {\mbox{\tt Beget}}
\def\Bta        {\mbox{\tt Beta}}
\def\betakfit   {\mbox{\tt BetaKfit}}
\def\cornelius  {\mbox{\tt Cornelius}}
\def\evtgen     {\mbox{\tt EvtGen}}
\def\euclid     {\mbox{\tt Euclid}}
\def\fitver     {\mbox{\tt FitVer}}
\def\fluka      {\mbox{\tt Fluka}}
\def\fortran    {\mbox{\tt Fortran}}
\def\gcalor     {\mbox{\tt GCalor}}
\def\geant      {\mbox{\tt GEANT}}
\def\gheisha    {\mbox{\tt Gheisha}}
\def\hemicosm   {\mbox{\tt HemiCosm}}
\def\hepevt     {\mbox{\tt{/HepEvt/}}}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}}
\def\minuit     {\mbox{\tt Minuit}}
\def\objegs     {\mbox{\tt Objegs}}
\def\paw        {\mbox{\tt Paw}}
\def\Root       {\mbox{\tt Root}}
\def\squaw      {\mbox{\tt Squaw}}
\def\stdhep     {\mbox{\tt StdHep}}
\def\trackerr   {\mbox{\tt TrackErr}}
\def\turtle     {\mbox{\tt Decay~Turtle}}

